Adversarial training in communication constrained federated learning

Federated learning enables model training over a distributed corpus of agent data. However, the trained model is vulnerable to adversarial examples, designed to elicit misclassification. We study the feasibility of using adversarial training (AT) in the federated learning setting. Furthermore, we do so assuming a fixed communication budget and non-iid data distribution between participating agents. We observe a significant drop in both natural and adversarial accuracies when AT is used in the federated setting as opposed to centralized training. We attribute this to the number of epochs of AT performed locally at the agents, which in turn effects (i) drift between local models; and (ii) convergence time (measured in number of communication rounds). Towards this end, we propose FedDynAT, a novel algorithm for performing AT in federated setting. Through extensive experimentation we show that FedDynAT significantly improves both natural and adversarial accuracy, as well as model convergence time by reducing the model drift.

==> Adversarial training in communication constrained federated learning/abstract.tex <==
% \begin{abstract}
% Federated learning is a distributed machine learning approach, which enables multiple parties to learn a joint model while keeping their data private. Adversarial training is a defense against test-time adversaries, wherein the network is trained on adversarial examples.
% Projcted Gradient Descent (PGD) based adversarial training has become one of the most prominent defense against adversarial attacks. In this paper, we explore the problem of distributed adversarial training to learn robust models in the federated setting. We propose our algorithm AdvFL (Adversarial Federated Learning) and support it with extensive experiments on both IID and NonIID data distributions for the Cifar10 dataset. We do a SVCCA analysis of the local models to highlight the impact of model drift in the NonIID data partition setting and methods to address the drift. 
% \end{abstract}

\begin{abstract}
    Federated learning enables model training over a distributed corpus of agent data. However, the trained model is vulnerable to adversarial examples -- designed to elicit misclassification. %Recently, adversarial training (AT) has emerged as the method of choice for training robust neural networks. 
    We study the feasibility of using adversarial training (AT) in the federated learning setting. Furthermore, we do so assuming a fixed communication budget and non-iid data distribution between participating agents. 
    %Using natural and adversarial accuracies for centralized clean training as baseline, we observe a higher drop in both accuracies when AT is used in the federated setting as opposed to centralized training.
    We observe a significant drop in both natural and adversarial accuracies when AT is used in the federated setting as opposed to centralized training. We attribute this to the number of epochs of AT performed locally at the agents, which in turn effects (i) \emph{drift} between local models; and (ii) convergence time (measured in number of communication rounds). Towards this end, we propose \feddynat -- a novel algorithm for performing AT in federated setting.
    Through extensive experimentation we show that \feddynat significantly improves both natural and adversarial accuracy, as well as model convergence time by reducing the model drift.
\end{abstract}

==> Adversarial training in communication constrained federated learning/challenges.tex <==
%\section{Challenges with adversarial training in federated setting}
\section{Impact of adversarial training on federated model performance}
\label{sec:challenges}
In this section, we empirically outline the primary challenges in adopting \at to federated setting. These challenges provide useful insights and motivate our proposed solution. We use \fedavg as our baseline fusion algorithm and compare the relative impact on performance due to \fedavgat.  
% \textcolor{red}{let's discuss how we should name 3.1 and 3.2. Do both of them are due to non-iid or accuracy is due to non-iid and communication overhead is even for iid or just non-iid?}

\subsection*{Datasets and model architecture for evaluation}
\label{subsec:data}
We conduct our evaluation with two datasets: CIFAR-10~\cite{cifar10} and EMNIST-Balanced~\cite{cohen2017emnist}. We use Network-in-Network (NIN)~\cite{lin2014network} and VGG-9 network~\cite{simonyan15} for training on the CIFAR-10 dataset.
For experiments with EMNIST-Balanced, we use a network with two convolution layers followed by two fully connected layers. We refer to this model as EMNIST-M in subsequent sections.

%\subsection{Impact of non-iid data}
\subsection{Increased drop in natural and adversarial accuracy with federated \at and non-iid data}
\label{subsec:non-iid}
In federated learning deployments, data partitions across clients invariably exhibit non-iid behavior \cite{mcmahan2016communicationefficient}. Thus, we begin by investigating the effect of adversarial training with non-iid data. 
Details for the data partition strategy for non-iid data can be found in Section.~\ref{non-iid split} 
Table~\ref{Adversarial_challenge} reports the performance of \fedavgat for both natural training and adversarial training for all the three models. The number of local training epochs, $E=1$. We also report results for centralized training (entire dataset available at the training site) for better comparison.

First, we observe that adversarial training with iid data distribution leads to performance that is close to that of centralized setting for all the three models. Second, as has been indicated in prior work~\cite{shoham2019overcoming}, we validate that using \fedavg with non-iid data, leads to a drop in accuracy even for natural training. However, as the main focus of our paper, we note a much larger drop in both natural and adversarial accuracies when performing adversarial training on non-iid data when compared to iid data. It is most severe for EMNIST-M model, where the adversarial accuracy drops from 72\% in the centralized setting to 58\%.

%Write about data augmentation?? with EMNIST-M
%Interestingly, the drop in natural accuracy is negligible. 

\begin{table}[!ht]
\small
\centering
% \begin{adjustwidth}{}{}
% \begingroup
\setlength{\tabcolsep}{3pt}
\begin{tabular}{p{1pt}ccccc}
\multicolumn{5}{c}{} \\
\cline{2-6}
 &  & & NIN & VGG & EMNIST-M \\
 \cline{2-6}
& Natural & Centralized & (88\%, 0\%) & (91\%, 0\%) & (87\%, 0\%) \\ [-0.05in]
&& iid & (87\%, 0\%) & (90\%, 0\%) & (86.5\%, 0\%)
 \\ [-0.05in]
&& non-iid & (78.5\%, 0\%) & (86\%, 0\%) & (82.5\%, 0\%) \\ \cline{2-6}
& Adversarial & Centralized & (75\%, 42\%) & (75\%, 44\%) & (84.5\%, 72\%) \\ [-0.05in]
&& iid & (74.5\%, 42\%) & (75, 44\%) & (84\%, 72\%)\\ [-0.05in]
&& non-iid & (67\%, 36\%) & (68.5\%, 36\%) & (84\%, 58\%)\\ 
\cline{2-6}
\end{tabular}
% \endgroup
% \end{adjustwidth}
\caption{\small Performance for natural and adversarial training for centralized and \fedavgat with K=5 clients. The performance is reported as a tuple: (natural accuracy, adversarial accuracy).}
\label{Adversarial_challenge}
\end{table}

We hypothesize increased model drift with non-iid data as the reason for the significant reduction in model performance with \fedavgat. Model drift refers to models learning very different representations of the data. At the start of a round, every client begins local adversarial training with the same model weights. However, the generated adversarial examples depend on both the local samples and the local model. As the local training progresses, the adversarial examples at the clients can become highly tuned towards the local data and model and may differ a lot from adversarial examples generated at other clients. Hence the models which are trained on these samples can exhibit significant drift. We validate our hypothesis and evaluate model drift in detail using SVCCA~\cite{raghu:svcca}  in Section~\ref{subsec:svcca}.

\subsection{Increased communication overhead} \label{sec:communication_overhead_section}
In this section, we study the effect of adversarial training on the convergence rate of the global model.
The convergence plots for \fedavg and \fedavgat on non-iid data between $K=5$ clients, with $E=1$ are shown in Fig.~\ref{fig:communication_challenge}. While \fedavg converges within $300$ communication rounds, \fedavgat takes about $800$ rounds to converge. This highlights that adversarial training requires more communication rounds compared to natural training in a federated setup. With faster compute infrastructure at the clients, increased communication cost is often the primary bottleneck for training of the models in a federated setting. 

% \textcolor{red}{AV: We observe this behaviour both 
% for iid as well as non-iid data distributions.}

%A slower convergence rate, implies greater number of rounds leading to larger communication overhead (due to update sharing).

%Reducing the convergence time and maintaining model accuracy, while performing \at in federated setting, is thus the other focus of this work.

%\setlength\belowcaptionskip{-1.7\baselineskip}
\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{aaaitoolkit/Challenge_communication_overhead.png} 
    \caption{\centering \small Accuracy vs communication round plot for \fedavg (natural training) and \fedavgat with 5 clients and non-iid data distribution using NIN.}
    \label{fig:communication_challenge}
\end{figure}

% \section{Impact on performance due to federation }
% %The key challenges with federated learning are non-iid data distribution across clients \cite{} and the associated communication overhead \cite{}.
% We evaluate the performance of \fedavgat and \fedcurvat and compare them with that of the centralized setting. We show that there is a notable drop in performance in the federated setting for adversarial training and and provide some insights into this drop by studying model drift among individual models at different clients.

% \subsection*{Dataset and model architecture for evaluation}
% We conduct our evaluation with two datasets: CIFAR-10 and EMNIST-Balanced \cite{cohen2017emnist}. 
% We use Network-in-Network (NIN) \cite{} and VGG-9 \cite{} \textcolor{red}{AV: references missing} for training on the CIFAR-10 dataset. 
% For experiments with EMNIST-Balanced, we use a network with two convolution layers followed by two fully connected layers. We refer to this model as EMNIST-M in subsequent sections. \textcolor{red}{AV: more details about this model can be found in ...}

% \subsection{Impact of non-iid data}
% In federated learning, data splits across clients are invariably non-iid \cite{mcmahan2016communicationefficient} so we are interested in adversarial training scenarios with non-iid data distribution. 
% \textcolor{red}{AV: please explain how did we create non-iid distribution, the split used etc. in detail}


% We report the performance of \fedavgat for both natural training and adversarial training in \cref{Adversarial_challenge}. 
% Note that adversarial training with an iid data distribution has performance close to that of the  centralized setting.
% \begin{table}[!ht]
% \scriptsize
% \centering
% \begin{adjustwidth}{}{}
% \begingroup
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{p{1pt}ccccc}
% \multicolumn{5}{c}{} \\
% \cline{2-6}
%  &  & & NIN & VGG & EMNIST-M \\
%  \cline{2-6}
% & Natural & Centralized & (88\%, 0\%) & (91\%, 0\%) & (87\%, 0\%) \\ [-0.05in]
% && iid & (87\%, 0\%) & (90\%, 0\%) & (86.5\%, 0\%)
%  \\ [-0.05in]
% && non-iid & (78.5\%, 0\%) & (86\%, 0\%) & (82.5\%, 0\%) \\ \cline{2-6}
% & Adversarial & Centralized & (75\%, 42\%) & (75\%, 44\%) & (84.5\%, 72\%) \\ [-0.05in]
% && iid & (74.5\%, 42\%) & (75, 44\%) & (-)\\ [-0.05in]
% && non-iid & (67\%, 36\%) & (68.5\%, 36\%) & (84\%, 58\%)\\ 
% \cline{2-6}
% \end{tabular}
% \endgroup
% \end{adjustwidth}
% \caption{\small Performance for natural and adversarial training for centralized and \fedavgat with $K=5$ clients. The performance is reported as a tuple: (natural accuracy, adversarial accuracy)}
% \label{Adversarial_challenge}
% \end{table}

% However, in case of non-iid data distribution, we notice a significant drop in both natural and adversarial accuracy for all the three models. We notice a sharp drop in adversarial accuracy for EMNIST-M from 72\% to 58\%.


% With non-iid data distribution, we expect the local models to drift apart from each other. The model drift refers to the weights of the locally trained models being very different across clients.  
% The adversarial samples used for training depend on the weights of the local model. 
% Local model drift results in diverse adversarial training examples across clients. These adversarial samples constitute effective attacks against the local model but may not be as effective against the global model. This can negatively impact the overall robustness of the global model. 

% \subsubsection{SVCCA analysis for understanding model drift with non-iid data} \label{svcca_challenge}
% SVCCA \cite{NIPS2017_7188} \cite{NIPS2018_7815} is a technique to compute the similarity between two network representations. We utilize this method to quantify the model drift between client models after they have trained on their respective local data. 
% A higher SVCCA score implies a lower model drift between the two models being compared. For a detailed explanation of SVCCA refer to \Cref{svcca}. 

% We compare SVCCA scores for \fedavg (natural training) vs \fedavgat (adversarial training) evaluated with E=50 in Fig.~\ref{fig:svcca_natural_adversarial.png}. The plots indicate that model drift worsens with adversarial training compared to natural training. 
% \begin{figure}[!ht]
% \includegraphics[width=1.0\columnwidth, left]{aaaitoolkit/svcca_natural_adversarial.png} 
%     \caption{SVCCA scores evaluated on 2 out of 5 clients for \fedavgat with E=50 for both adversarial training and natural training with NIN}
%     \label{fig:svcca_natural_adversarial.png}
% \end{figure}

% \subsection{Communication overhead}
% We study the convergence rates for \fedavg and \fedavgat with E=1 in \cref{communication_challenge}. While \fedavg converges within 300 communication rounds, \fedavgat takes 800 rounds for convergence.
% This highlights that adversarial training requires more communication rounds compared to natural training in a federated setup.

% With improved compute hardware at the clients, the communication cost per round is often the bottleneck. We need a mechanism to address the communication overhead for \fedavgat evaluated with E=1.  

% \begin{figure}[!ht]
% \includegraphics[width=1.0\columnwidth, left]{aaaitoolkit/Challenge_communication_overhead.png} 
%     \caption{Accuracy vs communication round for \fedavg (natural training) and \fedavgat with 5 clients and non-iid data distribution using NIN.}
%     \label{communication_challenge}
% \end{figure}

% % We try to solve a communication constrained adverserial training problem in the non-iid federated setting. We highlight the drop in performance with E=1 with a smaller communication budget in \cref{communication_challenge}. Communication budget is the maximum number of rounds of communication between server and clients. 


% % \begin{table}[!ht]
% % \small
% % \centering
% % \begin{adjustwidth}{}{}
% % \begingroup
% % \setlength{\tabcolsep}{3pt}
% % \begin{tabular}{p{1pt}cccc}
% % \multicolumn{3}{c}{} \\
% % \cline{2-4}
% %  & Communication Budget & NIN & VGG\\
% %  \cline{2-4}
% % & 50 rounds & (25\%, 20.5\%) & (47.3\%, 30.9\%) \\ [-0.05in]
% % & 100 rounds & (38.9\%, 26.2\%) & (57.8\%, 35.7\%) \\
% % [-0.05in]
% % & 600 rounds & (65\%, 36\%) & (68.5\%, 36\%) \\
% %  \cline{2-4}
% % \end{tabular}
% % \endgroup
% % \end{adjustwidth}
% % \caption{\small  The performance of the global model reported after 50, 100 and 600 rounds for 5client non-iid data split, trained with \fedavgat with E=1}
% % \label{communication_challenge}
% % \end{table}

==> Adversarial training in communication constrained federated learning/conclusion.tex <==
\section{Conclusion}
We proposed a novel algorithm for performing adversarial training of deep neural networks in a federated setting. We showed that federated setting specially with non-iid data distribution significantly affects the training performance due to model drift and takes much longer to converge as compared to natural training. We showed that the proposed algorithm is able to address the above challenges effectively and is able to get comparable or better accuracy in significantly lower number of rounds. 
%We were also able to corroborate our findings with SVCCA scores representing model drift across clients. 
Incorporating dynamic scheduling with more advanced model fusion techniques remains a topic of future research. 

==> Adversarial training in communication constrained federated learning/dependence_E.tex <==
\section{\feddynat Algorithm}
To address the twin challenges described in Section \ref{sec:challenges}, we propose a new algorithm, Federated Dynamic Adversarial Training (\feddynat). While prior work~\cite{Wang2019AdaptiveCS, spiridonoff2020local} have studied the tradeoff between communication overhead, and the convergence accuracy for natural training with iid data distribution. In this paper, we present this trade-off for adversarial training with non-iid data distribution.

\subsection{Influence of \mbox{$E$} on convergence} \label{influenceE_convergence}
To motivate \feddynat, we first discuss the \emph{sensitivity} of \at in a federated setting with respect to the number of local adversarial training epochs, $E$, between successive model aggregation. 
%So far we have used $E=1$ in all previous sections.
We vary the value of $E$ and study its impact on convergence speed as well as accuracy achieved.

The convergence plots for \fedavgat for $E = 1, 5$ and $20$ are presented in Fig.~\ref{fig:E_switch.png}. Setting $E=1$ leads to the best performance (for both natural and adversarial accuracy) but takes $800$ communication rounds to converge. The adversarial accuracy plots for $E=5$ and $E= 20$ converge much faster to almost the same accuracy as $E=1$ (after $800$ rounds), however, as training progresses the accuracy drops significantly. 
%as opposed to the plot for $E=1$ in the initial phase. However, these plots  fall off later to a lower accuracy for the adversarial accuracy. 

A higher value of $E$ is found to benefit the convergence speed for natural training as shown in \cite{mcmahan2016communicationefficient}. However, the fall in adversarial accuracy  with higher $E$ in the later phase of training can be explained with the findings in earlier studies \cite{pmlr-v97-wang19i,gupta20}. They show that the adversaries generated only in the later phase of the  training are  potent to the final model. A higher value of $E$ results in models drifting too much from each other due to non-iid data distribution (and hence the locally generated adversaries) but it starts to impact only in the later phase of the training. 

%As we discuss later in Section~\ref{subsec:svcca}, a higher value of $E$ results in higher model drift across client models specially in the later phase of training motivating the use of different values of $E$ during different phases of training.

%. This motivates us to use different values of $E$ in different phases of training.

%The adversarial accuracy plot in Fig.~\ref{fig:E_switch.png} (right column) shows the {\it crossover} points for  different plots. $E=20$ gives better adversarial accuracy in initial rounds. The first crossover point is where the plots for $E=20$ and $E=5$ intersect, following which $E=5$ gives better adversarial accuracy. The second crossover occurs at the intersection of the plots for $E=5$ and $E=1$, beyond which adversarial accuracy with $E=1$ is higher. 

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.5]{aaaitoolkit/E_switch_1_5_20.png}
    \caption{\centering \small The top row shows the accuracy vs.\ communication round plots with \fedavgat for $E=1, 20, 50$ on NIN. The bottom row is a zoomed version of the convergence plot, for first 100 communication rounds.}
    \label{fig:E_switch.png}
\end{figure}

\subsection{\fedcurvat improves performance over \fedavgat with higher $E$} \label{FedCurvature_improves_performance_highE_fedavg}


%We saw in Section.~\ref{sec:communication_overhead_section} that $E=1$ takes a lot of communication rounds to converge. We want to study if using a higher $E$ can result in faster convergence. 


%\subsection*{\fedcurvat improves performance over \fedavgat with higher $E$} \label{fedcurvature_improves_performance_higherE}
% We established previously that with \fedavgat there is significant model drift among local models in adversarial training.  
\fedcurv, as described in  Section.~\ref{fed_curvature}, has been shown to result in better performance as compared to \fedavg in the context of non-iid data distribution~\cite{shoham2019overcoming}. We evaluate performance of \fedcurvat on non-iid data and its dependency on $E$. 
Table~\ref{FedAvg_FedCurvature_non-iid_highE} compares the performance of \fedcurvat and \fedavgat for different values of $E$ for NIN, VGG and EMNIST-M models. 

We see a significant improvement in adversarial accuracy with \fedcurvat compared to \fedavgat. Further, the improvement increases as we increase $E$. We explain the dependence of model drift on $E$ in Section~\ref{subsec:svcca}. We attribute this improvement to \fedcurvat's regularized loss which helps in reducing model drift. 
Increased drift of local models affects the adversarial accuracy of the global model, reflected in \fedavgat results for $E=20$ and $E=50$.
\begin{table}[!hbt]
\centering
\small
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\begin{tabular}{p{1pt}cccrr}
\multicolumn{5}{c}{} \\
\cline{2-6}
 & Model & E & K & \fedavgat & \fedcurvat\\ 
 \cline{2-6}
& NIN & 20 & 2 & (62.1\%, 27.5\%) & (\textbf{66.6}\%, \textbf{33.5}\%)\\ [-0.05in]
&&& 5 & (67.1\%, 27.8\%) & (\textbf{66.6}\%, \textbf{31}\%) \\ [-0.05in]
&&& 10 & (61.6\%, 25.4\%) & (\textbf{62.4}\%, \textbf{30.1}\%) \\
 \cline{3-6}
&& 50 & 5 & (63.8\%, 24.5\%) & (\textbf{65.2}\%, \textbf{32}\%) \\ [-0.05in]
&&& 10 & (60.5\%, 21.7\%) & (\textbf{60.9}\%, \textbf{30.7}\%) \\
 \cline{2-6}
\end{tabular}
\quad
\begin{tabular}{p{1pt}cccrr}
\multicolumn{5}{c}{} \\
\cline{2-6}
 & Model & E & K & \fedavgat & \fedcurvat\\ 
 \cline{2-6}
& VGG & 20 & 2 & (60.2\%, 26.7\%) & (\textbf{67.1}\%, \textbf{30.5}\%)\\ [-0.05in]
&&& 5 & (67.7\%, 31.3\%) & (\textbf{68.3}\%, 31.3\%) \\ [-0.05in]
&&& 10 & (65.1\%, \textbf{29}\%) & (\textbf{65.6}\%, 28.3\%) \\
 \cline{3-6}
&& 50 & 5 & (64\%, 30.6\%) & (\textbf{66.8}\%, \textbf{32}\%) \\ [-0.05in]
&&& 10 & (\textbf{64}\%, 28.5\%) & (\textbf{64}\%, 28.7\%) \\
\cline{3-6}
\end{tabular}
\quad
\begin{tabular}{p{1pt}cccrr}
\multicolumn{5}{c}{} \\
\cline{2-6}
 & Model & E & K & \fedavgat & \fedcurvat\\ 
 \cline{2-6}
& EMNIST-M & 5 & 2 & (83.5\%, \textbf{60.5}\%) & (\textbf{84.5}\%, 60\%) \\ [-0.05in]
 &&& 5 & (80\%, 53.3\%) & (\textbf{81}\%, \textbf{55}\%) \\ [-0.05in]
 &&& 10 & (78.8\%, 48.4\%) & (\textbf{79.9}\%, \textbf{50}\%) \\
 \cline{3-6}
&& 20 & 2 & (80.3\%, 52.6\%) & (\textbf{83.1}\%, \textbf{56}\%)\\ [-0.05in]
&&& 5 & (74.1\%, 47\%) & (\textbf{78.6}\%, \textbf{50.4}\%)\\ [-0.05in]
&&& 10 & (72.8\%, 42.5\%) & (\textbf{76}\%, \textbf{45.7}\%) \\ 
 \cline{2-6}
\end{tabular}

\caption{\centering \small \fedavgat vs \fedcurvat for various $E$ values after 50 communication rounds, for NIN, VGG and EMNIST-M models.}
\label{FedAvg_FedCurvature_non-iid_highE}
\end{table}

% \begin{table}[!ht]
% \small
% \centering
% \begin{adjustwidth}{}{}
% \begingroup
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \begin{tabular}{p{1pt}cccc}
% \multicolumn{4}{c}{} \\
% \cline{2-5}
%  & E & K & \fedavgat & \fedcurvat\\ 
%  \cline{2-5}
% & 20 & 2 & (62.1\%, 27.5\%) & (66.6\%, 33.5\%)\\ [-0.05in]
% && 5 & (67.1\%, 27.8\%) & (66.6\%, 31\%) \\ [-0.05in]
% && 10 & (61.6\%, 25.4\%) & (62.4\%, 30.1\%) \\
%  \cline{2-5}
% & 50 & 5 & (63.8\%, 24.5\%) & (65.2\%, 32\%) \\ [-0.05in]
% && 10 & (60.5\%, 21.7\%) & (60.9\%, 30.7\%) \\
% \cline{2-5}
% \end{tabular}
% \endgroup
% \end{adjustwidth}
% \caption{\small \fedavgat vs \fedcurvat for E=20 \& E=50 for NIN with CIFAR10 dataset after 30 communication rounds.}
% \label{FedAvg_FedCurvature_non-iid_E=20}
% \end{table}

% \begin{table}[!ht]
% \small
% \centering
% \begin{adjustwidth}{}{}
% \begingroup
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \begin{tabular}{p{1pt}cccc}
% \multicolumn{4}{c}{} \\
% \cline{2-5}
%  & E & K & \fedavgat & \fedcurvat\\ 
%  \cline{2-5}
% & 20 & 2 & (60.2\%, 26.7\%) & (67.1\%, 30.5\%)\\ [-0.05in]
% && 5 & (67.7\%, 31.3\%) & (68.3\%, 31.3\%) \\ [-0.05in]
% && 10 & (65.1\%, 29\%) & (65.6\%, 28.3\%) \\
%  \cline{2-5}
% & 50 & 5 & (64\%, 30.6\%) & (66.8\%, 32\%) \\ [-0.05in]
% && 10 & (64\%, 28.5\%) & (64\%, 28.7\%) \\
% \cline{2-5}
% & 100 & 5 & (61.9\%, 27\%) & (67.1\%, 29.8\%) \\ [-0.05in]
% && 10 & (61.2\%, 27.8\%) & (62.9\%, 27\%) \\
% \cline{2-5}
% \end{tabular}
% \endgroup
% \end{adjustwidth}
% \caption{\small \fedavgat vs \fedcurvat for E=20, E=50 \& E=100 for VGG with CIFAR10 dataset after 30 communication rounds. }
% \label{FedAvg_FedCurvature_non-iid_E=20_VGG}
% \end{table}

% \begin{table}[!ht]
% \small
% \centering
% \begin{adjustwidth}{}{}
% \begingroup
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \begin{tabular}{p{1pt}cccc}
% \multicolumn{4}{c}{} \\
% \cline{2-5}
%  & E & K & \fedavgat & \fedcurvat\\ 
%  \cline{2-5}
%  & 5 & 2 & (83.5\%, 60.5\%) & (84.5\%, 60\%) \\ [-0.05in]
%  && 5 & (80\%, 53.3\%) & (81\%, 55\%) \\ [-0.05in]
%  && 10 & (78.8\%, 48.4\%) & (79.9\%, 50\%) \\
%  \cline{2-5}
% & 20 & 2 & (80.3\%, 52.6\%) & (83.1\%, 56\%)\\ [-0.05in]
% && 5 & (74.1\%, 47\%) & (78.6\%, 50.4\%)\\ [-0.05in]
% && 10 & (72.8\%, 42.5\%) & (76\%, 45.7\%) \\ 
%  \cline{2-5}
% \end{tabular}
% \endgroup
% \end{adjustwidth}
% \caption{\small  \fedavgat vs \fedcurvat for E=5 after 50 communication rounds and E=20 after 30 communication rounds on EMNIST dataset.}
% \label{EMNIST_non-iid_E=20}
% \end{table}




\input{fedcurvature_with_dynamicE}




==> Adversarial training in communication constrained federated learning/experimental_section.tex <==
\section{Experiments and Results}

\subsection{Experimental set-up}
We list here the implementation details, and the non-iid data partition strategy across clients. All experiments were conducted on a VM with eight Intel(R) Xeon(R) CPU E5-2690 v4 @ 2.60GHz CPUs and one NVIDIA V100 GPU. 

\subsubsection{non-iid data split} \label{non-iid split}
We conduct all our experiments with $K$ clients, $K \in \{2, 5, 10\}$. 
To achieve non-iid data distribution, we introduce skew in the data split. 
%split the data to achieve highly skewed data distribution across clients. 
Each client gets data corresponding to all the classes, but a majority of the data samples are from a subset of classes. We denote the set of majority classes at client $k$ as $M_{k}$ with ${\cal M}$ being the set of all classes in the dataset (e.g., for CIFAR-10 with 10 classes $|{\cal M}|=10$). ${\cal M}\setminus M_k$ will be the set of minority classes. We keep  $M_{k}$ as mutually exclusive across the clients.
We ensure that each client has roughly the same number of data samples.

We characterize the data split with a skew parameter $s$ which is a percentage of the aggregate data size corresponding to a class in ${\cal M}$. We first create $\{M_k\}$ by dividing all class labels in ${\cal M}$ equally among $K$ clients, i.e.$|M_k|=|{\cal M}|/K$. We then divide the total data across clients such that a client has $s\%$ of data for any class in ${\cal M} \setminus M_k$ and $(100-(K-1)*s)\%$ of data for a class in $M_k$. 
%For CIFAR10, $s$ values are $1,2,2$ for $K=2,5,10$
Table~\ref{skew_values} shows the skew values we have used for our non-iid data partitions.

\begin{table}[!ht]
\centering
\small
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\begin{tabular}{p{1pt}cccc}
\multicolumn{4}{c}{} \\
\cline{2-5}
 & Dataset & $K=2$ & $K=5$ & $K=10$ \\
 \cline{2-5}
& CIFAR-10 & 1\% & 2\% & 2\% \\
& EMNIST & 0.1\% & 0.1\% & 0.1\% \\
\cline{2-5}
\end{tabular}
\caption{\centering \small Skew parameter $s$ value used in our experiments.}
\label{skew_values}
\end{table}

% We give a overview of the data split with $K=2$ for both CIFAR10 and EMNIST dataset. We use similar techniques for $K=5, 10$ data split, details of which are in appenndix. 
% \begin{itemize}
%     \item CIFAR10: Each client has around 25000 training samples. We distribute 10 classes across 2 clients such that first client has 99\% of data with label $\in \numrange{0}{4}$ and 1\% data belonging to remaining 5 labels. The second client has 1\% data for labels $\in \{0,1,2,3,4\}$ and 99\% data belonging to remaining 5 labels
%     \item EMNIST-M: Each client has 65800 training samples. We distribute 47 classes across 2 clients such that first client has 99.9\% of data with label 
%     $\in \numrange{0}{23}$ and 0.1\% data belonging to remaining 23 labels. The second client has 0.1\% data for labels $\in \numrange{0}{23}$ and 99.9\% data belonging to remaining 5 labels
% \end{itemize}

\subsubsection{Implementation details}
All our models (NIN, VGG-9, and EMNIST-M) are implemented in Keras~\cite{chollet2015keras}. 
%We use the standard Network-in-Network~\cite{lin2014network} and VGG9 architectures~\cite{simonyan2015deep} for CIFAR-10. 
%The model for EMNIST data has 2 convolution layers with 32 filters each, followed by fully connected layer with 512 neurons, and a softmax layer for classification.
We use the PGD adversarial attack $A_{T, \epsilon, \alpha}$ which has 3 parameters: $T, \epsilon, \alpha$ (number of steps, ball size, step size). For CIFAR-10, we use $T=10, \epsilon= \frac{8}{255}, \alpha=\frac{2}{255}$. For EMNIST, we use  $T=10, \epsilon= \frac{3}{10}, \alpha=\frac{1}{20}$.
\at at each client is done with a batch size of $32$. For CIFAR-10, we use the SGD optimizer with a constant learning rate $=10^{-2}$ and momentum $=0.9$. For EMNIST, we use the Adam optimizer with a constant learning rate $=10^{-4}$.

To train the VGG network, we use data augmentation (random horizontal/vertical shift by 0.1 and horizontal flip). We do not use data augmentation for NIN and EMNIST-M networks.
We ignore all batch normalization \cite{10.5555/3045118.3045167} layers in the VGG architecture.


%\subsubsection{Tuning FedCurvature parameter $\lambda$}

\subsection{\feddynat results}
We compare \feddynat to \fedavgat and \fedcurvat baselines, both of which are run with a fixed value of $E$. For a given communication budget, we evaluate \fedavgat and \fedcurvat with various values of $E$ and report performance with $E$ resulting in best natural accuracy for the global model.
We report two observations in this section
\begin{itemize} [noitemsep,nolistsep]
    \item \feddynat outperforms \fedavgat, \fedcurvat for a fixed communication budget.
    \item \feddynat achieves similar performance as \fedavgat(E=1), 
    albeit in significantly lower number of communication rounds.
\end{itemize}

\subsubsection*{Results with varying $E$-schedule}
The dynamic $E$-schedule is defined by 3 parameters: the initial value $E_{0}$, decay rate $\gamma_{E}$ and decay frequency $F_{E}$ as described in Section~\ref{subsec:feddnyat}. We report the results for various combination of these parameters in  
Fig.~\ref{fig:E_schedule_FedDynAT}. The bottom row shows \fedcurvat results for 3 different fixed values of $E$. The top rows show the results for various configurations of the dynamic $E$ schedule. We notice an improved performance in both natural and adversarial accuracy with \feddynat with a smooth drop in $E$ compared to \fedcurvat with fixed $E$. 

%The bottom row further highlights the tradeoff with increasing $E$. $E=20$ has converged within the budget, resulting in a higher natural accuracy compared to $E=5$. However, the adversarial accuracy is lower due to increased model drift with a higher $E$.

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.5]{aaaitoolkit/E_schedule_FedDynAT.png} 
    \caption{\centering \small Performance of dynamic $E$ schedule with various parameter configurations. x-axis shows communication rounds and y-axis is the value of $E$ used in that round.}
    \label{fig:E_schedule_FedDynAT}
\end{figure}

\subsubsection{Accuracy with different communication budgets}
We set out to solve the adversarial training problem with non-iid data split in a communication constrained setting. We vary the communication buget i.e maximum number of communication rounds and demonstrate how \feddynat performs as compared to \fedavgat and \fedcurvat. We evaluate \fedavgat and \fedcurvat with multiple values of $E$ and report performance corresponding to the best natural accuracy of the global model.  Table~\ref{FedDynAT_NIN_100rounds} shows the results for Network-in-network model for CIFAR10 dataset and  Table~\ref{FedDynAT_EMNIST_20rounds} shows that of EMNIST-M model for EMNIST dataset. We defer results with VGG to the Supplement.



% The results with NIN with communication budget of 50 and 100 rounds are shown in Table~\ref{FedDynAT_NIN_100rounds}. 
% Similar results with EMNIST-M with a communication budget of 20 and 50 rounds are shown in Table~\ref{FedDynAT_EMNIST_20rounds}.

The convergence plot for \fedavgat, \fedcurvat and \feddynat with NIN with a budget of 50 rounds is presented in Fig.~\ref{fig:convergence_plot_50rounds}. Notice how the natural accuracy curves for all 3 algorthms converge to similar numbers but the adversarial accuracy with \feddynat is significantly better than \fedavgat and \fedcurvat. 
%$E=20$ gives the best natural accuracy performance with $K=5$ and $K=10$ clients within 50 communication rounds, consequently the adversarial accuracy with large $E$ is lower.

\noindent{\bf FedAvg fusion with dynamic $E$: } 
\feddynat uses the FedCurvature fusion algorithm. We consider another baseline where we replace the fusion algorithm with FedAvg and refer to it as \fedavgdynat.  
The results with NIN in Table~\ref{FedDynAT_NIN_100rounds} demonstrate that \feddynat  outperforms this baseline. In Section~\ref{FedCurvature_improves_performance_highE_fedavg} we established that \fedcurvat results in improvement over \fedavgat for higher $E$. A high $E_{0}$ for our E-schedule contributes to better eventual performance with \feddynat over \fedavgdynat.
We find \fedavgdynat performs similar to \feddynat for EMNIST dataset for the particular communication budget. 

\begin{table}[!ht]
\centering
\small
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\begin{tabular}{p{1pt}ccrrrr}
\multicolumn{6}{c}{} \\
\cline{2-7}
 & K & Budget & \fedavgat & \fedcurvat & \fedavgdynat & \feddynat \\
 \cline{2-7}
& 2 & 50 & (68.2\%, \textbf{38.5}\%) & (68.7\%, 37.8\%) & (67.2\%, 34.3\%) & (\textbf{68.4}\%, 38\%) \\ [-0.05in]
&& 100 & (70.0\%, 38\%) & (\textbf{71}\%, 37.5\%) & (67.2\%, 35.3\%) & (70.4\%, \textbf{38}\%) \\
\cline{2-7}
& 5 & 50 & (\textbf{67.1}\%, 27.8\%) & (66.6\%, 31\%) & (66.5\%, 34.8\%) & (66.6\%, \textbf{35.3}\%) \\ [-0.05in]
&& 100 & (64.9\%, 35\%) & (65.8\%, 35.2\%) & (66.8\%, 35\%) & (\textbf{66.8}\%, \textbf{35.9}\%) \\
\cline{2-7}
& 10 & 50 & (61.6\%, 25.4\%) & (61.9\%, 30.7\%) & (61.8\%, 30\%) & (\textbf{62.3}\%, \textbf{32.5}\%) \\ [-0.05in]
&& 100 & (61.6\%, 25.4\%) & (61.9\%, 30.7\%) & (61.9\%, 31.4\%) & (\textbf{62.6}\%, \textbf{33.3}\%) \\
 \cline{2-7}
\end{tabular}
\caption{\centering \small \feddynat performance on Network-in-network model for communication budgets of 50 and 100 rounds. We evaluate \fedavgat and \fedcurvat with $E=\{1, 5, 20\}$ and report the best individual performance.}
\label{FedDynAT_NIN_100rounds}
\end{table}

\begin{table}[!ht]
\centering
\small
\setlength{\tabcolsep}{2pt} % Default value: 6pt
\begin{tabular}{p{1pt}ccrrrr}
\multicolumn{6}{c}{} \\
\cline{2-7}
 & K & Budget &  \fedavgat & \fedcurvat & \fedavgdynat & \feddynat \\
 \cline{2-7}
& 2 & 20 & (83.5\%, 57.5\%) & (83.8\%, 60\%) & (84\%, 64\%) & (\textbf{84.5}\%, \textbf{64.2}\%) \\ [-0.05in]
&& 50 & (84.1\%, 65.5\%) & (84.1\%, 65.5\%) & (84\%, 64\%) &(\textbf{84.5}\%, \textbf{64.5}\%) \\
\cline{2-7}
& 5 & 20 & (78.4\%, 50.6\%) & (81\%, 55\%) & (82.1\%, \textbf{56.5}\%) & (\textbf{82.3}\%, 56.2\%) \\ [-0.05in]
&& 50 & (80.7\%, 54.3\%) & (81\%, 55\%) & (83.4\%, \textbf{59}\%) & (\textbf{83.6}\%, 58.3\%) \\
\cline{2-7}
& 10 & 20 & (75.8\%, 45.4\%) & (76.8\%, 45.8\%) & (78.9\%, \textbf{51.5}\%) & (\textbf{79.9}\%, 51.3\%) \\ [-0.05in]
&& 50 & (78.3\%, 47.5\%) & (79.9\%, 50\%) & (\textbf{81.9}\%, \textbf{54.8}\%) & (81.7\%, 54.7\%) \\
\cline{2-7}
\end{tabular}
\caption{\centering \small \feddynat performance on EMNIST-M compared to \fedavgat, \fedcurvat with a communication budget of 20 and 50 rounds. We evaluate \fedavgat and \fedcurvat with $E=\{1, 5, 20\}$ and report performance with $E$ resulting in best natural accuracy.}
\label{FedDynAT_EMNIST_20rounds}
\end{table}

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.5]{aaaitoolkit/convergence_plot_50rounds.png} 
    \caption{\centering \small Accuracy vs communication round for \fedavgat, \fedcurvat and \feddynat with NIN for a communication budget of 50 rounds.}
    \label{fig:convergence_plot_50rounds}
\end{figure}


\subsubsection{Convergence speed for \feddynat} \label{convergence_speed_section}
Figure~\ref{fig:convergence_plot_fedavg_E=1_FedDynAT} shows that convergence is much faster with \feddynat compared to \fedavgat(E=1) for both NIN and EMNIST-M. 
For reaching the same accuracy, with NIN, \feddynat converges in 100 communication rounds while \fedavgat takes 800 rounds to converge. Similarly, 
with EMNIST-M, \feddynat converges in 50 communication rounds while \fedavgat takes 150 rounds to converge.
Results for other values of $K$ are included in the appendix.

\begin{figure}[]
\includegraphics[width=1.0\columnwidth]{aaaitoolkit/convergence_plot_fedavg_E=1_FedDynAT.png} 
    \caption{\small Accuracy vs communication round plot for \feddynat and \fedavgat evaluated with E=1, on $K=5$ client non-iid data split with NIN and EMNIST-M.} %Notice that \feddynat converges after 100 communication rounds, showing similar performance as \fedavgat which converges after 800 rounds.}
    \label{fig:convergence_plot_fedavg_E=1_FedDynAT}
\end{figure}

\subsection{Understanding performance through model drift: A SVCCA-based Analysis }
\label{subsec:svcca}
\input{svcca_analysis}



% \begin{table}[!ht]
% 
% \centering
% \begin{adjustwidth}{}{}
% \begingroup
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \begin{tabular}{p{1pt}ccccc}
% \multicolumn{5}{c}{} \\
% \cline{2-6}
%  & K & \fedavgat & \fedcurvat & \fedavgat\_DynamicE & \feddynat \\
%  \cline{2-6}
% & 2 & (70.0\%, 38\%) & (71\%, 37.5\%) & (67.2\%, 35.3\%) & (70.4\%, 38\%) \\ [-0.05in]
% & 5 & (64.9\%, 35\%) & (65.8\%, 35.2\%) & (66.8\%, 35\%) & (66.8\%, 35.9\%) \\ [-0.05in]
% & 10 & (61.6\%, 25.4\%) & (62.4\%, 30.1\%) & (61.9\%, 31.4\%) & (62.6\%, 33.3\%) \\
%  \cline{2-6}
% \end{tabular}
% \endgroup
% \end{adjustwidth}
% \caption{\small \feddynat performance on NIN compared to \fedavgat, \fedcurvat with best static E with a communication budget of 100 rounds}
% \label{FedDynAT_NIN_100rounds}
% \end{table}


% \begin{figure}[htp]

%   \centering


%   \begin{tabular}{ccc}

%     % Requires \usepackage{graphicx}

%     \includegraphics[width=30mm]{aaaitoolkit/adaptiveE_iid.png} & 

%     \includegraphics[width=30mm]{aaaitoolkit/adaptiveE_iid.png}&

%     \includegraphics[width=30mm]{aaaitoolkit/adaptiveE_iid.png}\\

%     \includegraphics[width=30mm]{aaaitoolkit/adaptiveE_iid.png}&

%     \includegraphics[width=30mm]{aaaitoolkit/adaptiveE_iid.png}&

%     \includegraphics[width=30mm]{aaaitoolkit/adaptiveE_iid.png}\\

%   \end{tabular}
% \label{figur}\caption{equation...}
% \end{figure}

% \begin{table}[!ht]
% 
% \centering
% \begin{adjustwidth}{}{}
% \begingroup
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \begin{tabular}{p{1pt}ccccc}
% \multicolumn{5}{c}{} \\
% \cline{2-6}
%  & K & \fedavgat & \fedcurvat & \fedavgat\_DynamicE & \feddynat \\
%  \cline{2-6}
% & 2 & (68.2\%, 38.5\%) & (68.7\%, 37.8\%) & (67.2\%, 34.3\%) & (68.4\%, 38\%) \\ [-0.05in]
% & 5 & (67.1\%, 27.8\%) & (66.6\%, 31\%) & (66.5\%, 34.8\%) & (66.6\%, 35.3\%) \\ [-0.05in]
% & 10 & (61.6\%, 25.4\%) & (62.4\%, 30.1\%) & (61.8\%, 30\%) & (62.2\%, 32.6\%) \\
%  \cline{2-6}
% \end{tabular}
% \endgroup
% \end{adjustwidth}
% \caption{\small \feddynat performance on NIN compared to \fedavgat, \fedcurvat with best static E with a communication budget of 50 rounds}
% \label{FedDynAT_NIN_50rounds}
% \end{table}

==> Adversarial training in communication constrained federated learning/fedavg-adv-train.tex <==
\subsection{\fedavgat Algorithm} 
The first fusion algorithm we consider is Federated Averaging \cite{mcmahan2016communicationefficient} which is a widely used algorithm in federated learning.
%The loss function at client $k$ is given by:
%\[ \bm{write the expression} \]

%\cite{mcmahan2016communicationefficient} shows that when we start two models from the same random initialization and then train each independently on a different subset of the data, a naive parameter averaging of the 2 models works well. We show that a naive averaging of the models works well even for adversarial training. 

% \begin{figure}[!ht]
%     \centering
% \includegraphics[width=1.0\columnwidth]{aaaitoolkit/Common Initialization.png} 
%     \caption{The loss on the full CIFAR10 training set (on natural and adversarial samples) for models generated by averaging the parameters of two models $\theta$ and $\theta^{'}$ using $w \theta + (1 − w) \theta^{'}$ for 50 evenly spaced values $w \in [−0.2, 1.2]$. The models $\theta$ and $\theta^{'}$ were initialized with the same weights and adversarially trained using SGD on different small datasets. As we see from the figure, averaging the models produces a significant reduction in the loss on the total training set for both natural and adversarial samples much better than the loss of either parent model [{\textcolor{red} {What happens in case of non-iid?}}]}
%     \label{fig:common_initialization}
% \end{figure}

%With the Federated Averaging fusion from \href{Federated_adversarial_training_algo}, 
At the end of round $t$, each client sends its model parameters, $\theta^{t}_{k}$, back to server. The server performs a weighted average of the model parameters to obtain the aggregate model parameters $\theta^{t+1}$ for the next round as:
% $\theta^{t+1} = \frac{1}{|D|}\sum_{k}|D_k| \theta^{t}_{k}$
\begin{equation}
    \label{eqn:fedavgupdate}
    \theta^{t+1} = \frac{1}{|D|}\sum_{k}|D_k| \theta^{t}_{k}
\end{equation}

%\textcolor{red}{AV: shall we get into different amounts of data at different clients? I am afraid what implication it will have in term of different number of model updates at each client if we use same batch size. Does McMahan deal with that?}
% \subsubsection{Performance on IID data}
% We look at the performance of FedAvg Adversarial Training algorithm on CIFAR10 dataset partitioned across K clients in an IID fashion and compare it to an adversarially trained model in the centralized setting. We use the Network-in-Network \cite{lin2014network} architecture for all experiments.

% Tradeoff between communication rounds(value of E) and performance??
% \begin{figure}[!ht]
% \hspace*{-1cm}  
% \includegraphics[width=1.3\columnwidth, left]{aaaitoolkit/FedAvg_IID_E=1.png} 
%     \caption{We look at the performance of FedAvg adversarial training with varied number of clients in {2, 5, 10, 16} and a fixed value of local training epochs $E=1$. The x-axis is the communication round and the y-axis plots the test accuracy numbers for natural and adversarial samples. The takeaway observation from this figure is that convergence wrt communication rounds, slows down as the number of participating clients increase. However when run for sufficiently large number of communication rounds, the performance converges to the centralized adversarial training performance.}
%     \label{fig:FedAvg_IID_E=1.png}
% \end{figure}


% \begin{figure}[!ht]
% %\hspace*{-1cm}  
% \includegraphics[width=1.3\columnwidth, left]{aaaitoolkit/FedAvg_IID_E=20.png} 
%     \caption{We look at the performance of FedAvg adversarial training with varied number of clients in {2, 5, 10, 16} and a fixed value of local training epochs $E=20$. The x-axis is the communication round and the y-axis plots the test accuracy numbers for natural and adversarial samples. The takeaway observation is that having a higher $E$ speeds up the convergence wrt communication rounds, but converges to a sub-optimal model. The model at convergence is less robust compared to a model obtained with FedAvg adversarial training with a smaller $E=1$, as evident from the adversarial accuracy plot.   \textcolor{red}{It's not clear from the plots above, in fact, it looks like the convergence is happening at much faster rate as opposed to E=1 but with a much lower accuracy! We may need to run with more number of rounds to conclude.}
%     } 
%     \label{fig:FedAvg_IID_E=20.png}
% \end{figure}


% \subsection{Performance on Non-IID data}
% We see that FedAvg adversarial training converges to centralized adversarial training performance when run sufficiently long. We now analyse the impact of Non-IID data on the model convergence and eventual performance. Non-IID data setting is when all the clients do not have a similar class distribution in their local data. This has been studied for federated learning as in \cite{zhao2018federated}, \cite{kim2020on}. 

% \begin{table}[!ht]
% \scriptsize
% \centering
% \begin{tabular}{p{1pt}ccccc}
% \multicolumn{5}{c}{} \\
% \cline{2-6}
%  &  & & 2 clients & 5 clients & 10 clients \\ 
%  \cline{2-6}
% & E=1 & Natural Accuracy & 70\% & 56\% & -\% \\ [-0.05in]
% && Adversarial Accuracy & 40\% & 34\% & -\% \\ 
% \cline{2-6}
% & E=20 & Natural Accuracy & 64\% & 66\% & 62\% \\ [-0.05in]
% && Adversarial Accuracy & 28\% & 27\% & 24\% \\ 
% \cline{2-6}
% & E=50 & Natural Accuracy & -\% & 63.8\% & 60.5\% \\ [-0.05in]
% && Adversarial Accuracy & -\% & 24.5\% & 21.7\% \\ 
%  \cline{2-6}

% \end{tabular}
% \caption{\small FedAvg Adversarial Training performance on NonIID data}
% \label{FedAvg_NonIID_E=20}
% \end{table}

% \begin{figure}[!ht]
% \hspace*{-1cm}  
% \includegraphics[width=1.3\columnwidth, left]{aaaitoolkit/FedAvg_NonIID_E=20.png} 
%     \caption{We look at the performance of FedAvg adversarial training for NonIID data with varied number of clients in {2, 5, 10, 16} and a fixed value of local training epochs $E=20$. The x-axis is the communication round and the y-axis plots the test accuracy numbers for natural and adversarial samples. The number of communication rounds The takeaway observation from this figure is that convergence wrt communication rounds, slows down as the number of participating clients increase. However when run for sufficiently large number of communication rounds, the performance converges to the centralized adversarial training performance.}
%     \label{fig:FedAvg_NonIID_E=20.png}
% \end{figure}


%show it works for E=1 and E=20 

%\textcolor{red}{Supriyo: Not clear what we are saying in this section: Are we saying that for IID-data, FedAvg Adv Training, converges to the centralized Adv Training when trained for longer. Using adaptive E, we can get the same accuracy in fewer communication rounds. What are we saying about Non-IID data? Table 2 is showing that performance of Adversarial Accuracy is much worse compared to Natural accuracy. Should we call Natural Accuracy as Clean accuracy?}

==> Adversarial training in communication constrained federated learning/fedcurv-adv-train.tex <==
\subsection{\fedcurvat Algorithm} 
\label{fed_curvature}
With non-iid data distribution between clients, local models tend to drift apart and inhibit learning using \fedavg. In \fedcurv~\cite{shoham2019overcoming}, a penalty term is added to the local training loss, compelling all local models to converge to a shared optimum.
% The approach draws inspiration from Elastic Weight Consolidation (EWC)~\cite{kirkpatrick2016overcoming}, a Lifelong Learning algorithm, designed to avoid catastrophic forgetting effects. 

At any client $k$, the loss function used for training $\Lagr(f_{\theta}(\Tilde{x}_{k}), y_{k})$ comprises of two components: 

\noindent{1.} Training loss on local data, $L_{k}(\theta)$.

\noindent{2.} Regularization loss, $R_k(\theta)$, given by:
  \[R_k(\theta) = \small \sum\limits_{j \in K \setminus k} (\theta - \hat{\theta}_{t-1,j}) \text{diag}(\hat{\mathcal{I}}_{t-1,j}) (\theta - \hat{\theta}_{t-1,j})\].

At the beginning of round $t$, starting from the initial point $\theta^t$ given by Eqn.(\ref{eqn:fedavgupdate}), each node optimizes $L_{k}(\theta) + \lambda R_k(\theta)$. 
At end of round $t$, client $j$ sends its local model weights $\hat{\theta}_{t,j}$ and the diagonal of Fisher Information Matrix $\hat{\mathcal{I}}_{t,j}$, evaluated on its local dataset and local model weights. 
$\lambda$ is the regularization hyperparameter which balances the tradeoff between local training, and model drift from the local client weights at the end of previous round.

% \subsection{\fedcurvat algorithm} 
% \label{fed_curvature}
% % loss function 
% % performance results with non-iid
% %  E=20
% % Compare with E=20 results for FedAvg adv. Comment that E=1 Fedcurv does not work. 
% With non-iid data distribution between clients, local models tend to drift apart and inhibit learning using \fedavg. In \fedcurv~\cite{shoham2019overcoming}, a penalty term is added to the cross-entropy loss -- training with regularization loss curtails the local model drift and results in much effective federated learning. The approach draws inspiration from Elastic Weight Consolidation (EWC)~\cite{kirkpatrick2016overcoming}, a Lifelong Learning algorithm, designed to avoid catastrophic forgetting effects. 

% %\subsection{Loss Function}
% %Following from the adversarial training framework in \Cref{Federated_adversarial_training_algo}, each client receives the global model weights at the beginning of each round. It then proceeds to train the model on adversarially generated samples from its local dataset. The set of all K clients is denoted by $S = {1 ... K}$ 
% At any client $k$, the loss function used for training $\Lagr(f_{\theta}(\Tilde{x}_{k}), y_{k})$ comprises of two components: 

% \noindent{1.} Training loss on local data, $L_{k}(\theta)$.

% \noindent{2.} Regularization loss, $R_k(\theta)$, given by:
%   \[R_k(\theta) = \small \sum\limits_{j \in K \setminus k} (\theta - \hat{\theta}_{t-1,j}) \text{diag}(\hat{\mathcal{I}}_{t-1,j}) (\theta - \hat{\theta}_{t-1,j})\].

% At the beginning of round $t$, starting from the initial point $\theta^t$ given by (\ref{eqn:fedavgupdate}), each node optimizes $L_{k}(\theta) + \lambda R_k(\theta)$. 
% At end of round $t$, client $j$ sends its local model weights $\hat{\theta}_{t,j}$ and the diagonal of Fisher Information Matrix $\hat{\mathcal{I}}_{t,j}$, evaluated on its local dataset and local model weights. 
% Here $\lambda$ is the regularization hyperparameter which balances the tradeoff between local training and model drift from the local client weights at end of previous round.

% \subsection{FedCurvature results}

% \begin{table}[!ht]
% \scriptsize
% \centering
% \begin{adjustwidth}{}{}
% \begingroup
% \setlength{\tabcolsep}{3pt} % Default value: 6pt
% \hspace*{-0.35cm}
% \begin{tabular}{p{1pt}cccccc}
% \multicolumn{6}{c}{} \\
% \cline{2-7}
%  &  & & \thead{\scriptsize FedAvg \\ \scriptsize Natural Acc} & \thead{\scriptsize  FedAvg \\ \scriptsize  Adversarial Acc} & \thead{\scriptsize FedCurvature \\ \scriptsize Natural Acc} & \thead{\scriptsize FedCurvature \\ \scriptsize Adversarial Acc}\\ 
%  \cline{2-7}
% & \scriptsize IID, E=20 & K=2 & 74.2\% & 39.7\% & 74.3\% & 40.0\% \\ [-0.05in]
% && K=5 & 72.6\% & 37.2\% & 72.4\% & 38.6\%\\ [-0.05in]
% && K=10 & 70.6\% & 33.4\% & 70.5\% & 35.7\%\\ [-0.05in]
% && K=16 & 70.5\% & 30.0\% & 69.7\% & 34.7\% \\ 
% \cline{2-7}
% & \scriptsize NonIID, E=20 & K=2 & 62.1\% & 27.5\% & 66.6\% & 33.5\%\\ [-0.05in]
% && K=5 & 67.1\% & 27.8\% & 66.6\% & 31\%\\ [-0.05in]
% && K=10 & 61.6\% & 25.4\% & 62.4\% & 30.1\%\\
%  \cline{2-7}
%  & \scriptsize IID, E=50 & K=5 & 70.6\% & 33.8\% & 72\% & 38.2\% \\ [-0.05in]
% && K=10 & 68.6\% & 31.2\% & 69.8\% & 35.9\% \\ [-0.05in]
% && K=16 & 67.6\% & 29\% & 67.1\% & 35.9\% \\ 
% \cline{2-7}
% & \scriptsize NonIID, E=50 & K=5 & 63.8\% & 24.5\% & 65.2\% & 32\% \\ [-0.05in]
% && K=10 & 60.5\% & 21.7\% & 60.9\% & 30.7\% \\ [-0.05in]
% \end{tabular}
% \endgroup
% \end{adjustwidth}
% \caption{\small FedCurvature vs FedAvg adversarial training for E=20 \& E=50. 
% Write observations here}
% \label{FedAvg_NonIID_E=20}
% \end{table}

% \begin{figure}[!ht]
% \hspace*{0.1cm}  
% \begin{minipage}[b][0.24\textwidth][c]{0.5\textwidth}
%     \includegraphics[width=\textwidth]{aaaitoolkit/FedCurvature_NonIID_E=20_K=2.png}
%     K=2, E=20
% \end{minipage}

% \begin{minipage}[b][0.24\textwidth][c]{0.5\textwidth}
%     \includegraphics[width=\textwidth]{aaaitoolkit/FedCurvature_NonIID_E=20_K=5.png}
%     K=5, E=20
% \end{minipage}

% % \begin{minipage}[b][0.24\textwidth][c]{0.23\textwidth}
% %     \includegraphics[width=\textwidth]{aaaitoolkit/FedCurvature_NonIID_E=20_K=2.png}
% %     K=2, E=20
% % \end{minipage}
  
% % \includegraphics[width=0.43\columnwidth, left]{aaaitoolkit/FedCurvature_NonIID_E=20_K=2.png} 
% % %\caption{FedCurvature vs FedAvg adversarial training for $K=2$ clients}
% % \label{fig:FedCurvature_NonIID_E=20_K=2}
% % \includegraphics[width=0.43\columnwidth, right]{aaaitoolkit/FedCurvature_NonIID_E=20_K=2.png} 
% % %\caption{FedCurvature vs FedAvg adversarial training for $K=2$ clients}
% % \label{fig:FedCurvature_NonIID_E=50_K=2}
% \hspace*{-1cm}  
% \includegraphics[width=0.5\columnwidth, left]{aaaitoolkit/FedCurvature_NonIID_E=20_K=5.png} 
% \caption{FedCurvature vs FedAvg adversarial training for $K=5$ clients}
% \label{fig:FedCurvature_NonIID_E=20_K=5}
% \hspace*{-1cm}  
% \includegraphics[width=1.0\columnwidth, left]{aaaitoolkit/FedCurvature_NonIID_E=20_K=10.png} 
% \caption{FedCurvature vs FedAvg adversarial training for $K=10$ clients}
% \label{fig:FedCurvature_NonIID_E=20_K=10}
% \end{figure}



==> Adversarial training in communication constrained federated learning/fedcurvature_with_dynamicE.tex <==
\subsection{Our algorithm : \feddynat}
\label{subsec:feddnyat}
% In Section.~\ref{influenceE_convergence}, we discuss the tradeoff between the convergence accuracy and the number of communication rounds to convergence when varying $E$.
% In Section.~\ref{FedCurvature_improves_performance_highE_fedavg}, we show that \fedcurvat outperforms \fedavgat for high values of $E$, and the improvement increases with $E$. 

% A high value of $E$ leads to large model drift affecting the adversarial accuracy of the global model. A low value of $E$ results in a higher adversarial accuracy at convergence but converges slowly, resulting in high communication cost.
The experiments (in Sections.~\ref{influenceE_convergence} and \ref{FedCurvature_improves_performance_highE_fedavg}) lead to two primary observations: (i) A high value of $E$ leads to large model drift affecting the adversarial accuracy of the global model. A low value of $E$ results in a higher adversarial accuracy at convergence but converges slowly, resulting in high communication cost. (ii) \fedcurvat outperforms \fedavgat for high values of $E$, and the improvement increases with $E$.

We combine the insights in our algorithm \feddynat, which follows a dynamic schedule for the number of local training epochs at each round. The training starts with a high value of $E = E_{0}$, and decays its value every $F_{E}$ rounds by a decay factor of $\gamma_{E}$. Further, we use \fedcurv as the fusion algorithm (but it does not preclude the use of \fedavg for fusion). Details of the algorithm are outlined in Algorithm ~\ref{FedDynAT_algo}.
% \bo{if you need space, you may put algo 1 in appendix and keep algo 2. However, it would be good to list out the challenges of directly applying algo 1 at beginning of sec 4, and lead to the later subsections on how to address them with overview.}

\begin{algorithm}[]
\small
%\SetAlgoLined
\caption{\small \textbf{\feddynat}}
 \label{FedDynAT_algo}
 \begin{algorithmic}
 \STATE {\bfseries Input:} number of clients: $K$, number of communication rounds: $R$, PGD Attack: $A_{T, \epsilon, \alpha}$, Initial model weights: $\theta^{0}$, Local training epochs at start: $E_{0}$, Decay rate: $\gamma_{E}$, 
 Decay frequency: $F_{E}$
 
 \FOR{$t=0$ {\bfseries to} $R-1$}
 \STATE $E_{t}= \ceil*{E_{0}*\gamma_{E}^{\floor*{\frac{t}{F_{E}}}}} $ \\
 %\STATE \COMMENT{ Client k does adversarial training on its local dataset} \\
 \STATE Server sends $\theta^{t}$ to all devices \\
 \FOR{client $k=0$ {\bfseries to} $K-1$}
  \STATE $\theta^{t}_{k}$ = \at($E_t$, $\theta^{t}$, $A_{T, \epsilon, \alpha}$) \\
  \STATE Send $\theta^{t}_{k}$ back to server \\
 \ENDFOR
 \STATE \COMMENT {Server performs aggregation over agent updates} \\ $\theta^{t+1} = \fedcurv(\theta_1^{t}, \ldots, \theta_{K}^{t})$ \\
 \ENDFOR
  \end{algorithmic}
\end{algorithm}

==> Adversarial training in communication constrained federated learning/federated_adversarial_training.tex <==
\section{Adversarial Training in Federated Setting}

%  We consider adversarial training in the scenario where there are $K$ clients, each having their share of the training data $D_k$. Let $D_k\thicksim{\cal F}_k$ and $D (=\bigcup_{k=1}^K D_k) \thicksim {\cal F}$. 
Following~\cite{madry2018towards}, we define centralized adversarially trained model parameters,  $\hat{\theta}$, as a solution to the following min-max problem:
 \begin{equation}
 \label{eqn:fedat0}
 \min_{\theta} \rho(\theta); \ \ \ 
 \rho(\theta) =  \E_{(x,y) \thicksim {\cal F}} [\max_{\norm{\Tilde{x}-x}_{\infty} \leq \epsilon} \Lagr(f_{\theta}(\Tilde{x}), y)]
 \end{equation}
 where $f_{\theta}$ is the model parameterized by $\theta$ and $\Tilde{x}$ is an $l_{\infty}$ adversarial sample, within $\epsilon$-ball of the benign sample $x$, with class label $y$.
 
 %$\epsilon$-ball $l_{\infty}$ adversarial sample of benign sample $x$ with class label $y$.
 \noindent{\bf Problem Formulation:} We consider adversarial training between $K$ clients, each having their share of the training data $D_k\thicksim{\cal F}_k$ and $D (=\bigcup_{k=1}^K D_k) \thicksim {\cal F}$.
 %In a federated setting a client's local data cannot be shared, we cannot expect to have the total training data $D$ at a centralized location. 
 Our objective is to train a joint machine learning model {\it without any exchange} of training data between clients.
 Motivated by our initial observations in (Figure~\ref{fig:feasibility}) we investigate adversarial training in federated environment as a combination of local adversarial training at individual clients followed by periodic synchronization and aggregation of model parameters at a trusted server. The aggregation, achieved by {\it fusing} the model weights of individual clients, results in a {\it global model}. The expectation is that after a sufficiently large number of aggregation rounds $t_0$,  this global model  will be an approximate solution to \eqref{eqn:fedat0}, i.e., $\rho(\theta^{t_0}) \approx \rho(\hat{\theta})$, providing robustness to adversarial attacks at all clients. 
 
Let $\theta_k^{t} \in \mathbb{R}^{n}$ be the model parameters at client $k = 1, \ldots, K$ at the beginning of round $t$. The aggregation of model weights is achieved using a fusion operator $F:\mathbb{R}^{K \times n} \rightarrow \mathbb{R}^{n}$. We denote the fusion output at the end of round $t$ as $\theta^{t+1}$. A training round $t$ involves $E_t$ epochs of adversarial training using local data at each agent. Thus, $\theta_k^t$ is a solution to the following min-max problem obtained over $E_t$ epochs with initial value $\theta_k^{t}=\theta^{t}$:
\begin{eqnarray}
\min_{\theta} \rho_k(\theta); \ \rho_k(\theta) & = &  \E_{(x,y) \in D_{k}} [\max_{\norm{\Tilde{x}-x}_{\infty} \leq \epsilon} \Lagr(f_{\theta}(\Tilde{x}), y)] \nonumber \\ 
\mbox{ and } \theta^{t+1} & = & F(\theta_1^t, \theta_2^t, \ldots, \theta_K^{t})
\label{eqn:advfed}
\end{eqnarray}
%and $\theta^{t+1} = F(\theta_1^t, \theta_2^t, \ldots, \theta_K^{t})$.

%\textcolor{red}{AV: we need to fix the notations here, specifically the subsript and superscript for $\theta$. Also we are using $t$ both as index and constant, e.g. above in sentence "after t rounds of fusion"}
%  $$ \min_{\theta} \rho_k(\theta); \ \ \ \rho_k(\theta) =  \E_{(x,y) \in D_{k}} [\max_{\norm{\Tilde{x}-x}_{\infty} \leq \epsilon} \Lagr(f_{\theta}(\Tilde{x}), y)]$$
%  and $\theta^{t+1} = F(\bm{\theta_{k}^{t}})$.


%  Let $\theta_k^t$ be the model weights at client $k$ and $\theta$ be the global model obtained by a fusion algorithm. We denote the fusion as an operator $F:\mathbb{R}^k \rightarrow \mathbb{R}$ mapping $\bm{\theta}$ to $\theta$, where $\bm{\theta} = \{\theta_k\}$. We denote the corresponding model parameters at the end of round $t$ of local adversarial training as $\theta_k^t$ and the fusion output as $\theta^{t+1}$. Each local training round involves $E_k$ epochs of adversarial training using local data of client $k$. Thus $\theta_k^t$ is a solution to the following min-max problem obtained over $E_k$ epochs with initial value $\theta_k^{t-1}=\theta^{t-1}$:
%  $$ \min_{\theta} \rho_k(\theta); \ \ \ \rho_k(\theta) =  \E_{(x,y) \in D_{k}} [\max_{\norm{\Tilde{x}-x}_{\infty} \leq \epsilon} \Lagr(f_{\theta}(\Tilde{x}), y)]$$
%  and $\theta^{t+1} = F(\bm{\theta_{k}^{t}})$. 

%FedAT (Algorithm~\ref{algo:FedAT}) is our general federated adversarial training 
The general optimization framework for solving Eqn.\eqref{eqn:advfed} is given in Algorithm~\ref{algo:FedAT}.%\textcolor{red}{equation number (2) should be for both the equations above also formatting on the second line of (2)} 
We consider two specific implementations of the fusion algorithm: Federated Averaging Adversarial Training (\texttt{FedAvgAT}) and Federated Curvature Adversarial Training (\texttt{FedCurvAT}). These fusion algorithms differ in the choice of their loss function $\Lagr$ and fusion operator $F$. \texttt{FedAvgAT} uses the cross-entropy loss function and weighted average of model weights as fusion operation. \texttt{FedCurvAT} in turn employs regularized loss function and an extended fusion involving the model weights and some auxiliary parameters. 
%\textcolor{red}{how is the FedCuv different from FedAvg? It's not described anywhere. only the loss function is explained}
\begin{algorithm}[]
\small
%\SetAlgoLined
\caption{\small \textbf{Federated adversarial training framework}}
 \label{Federated_adversarial_training_algo}
 \begin{algorithmic}
 \STATE {\bfseries Input:} number of clients: $K$, number of communication rounds: $R$, PGD Attack $A_{T, \epsilon, \alpha}$ with 3 parameters: $T, \epsilon, \alpha$(number of PGD steps, perturbation ball size, step size) , number of local training epochs per round: $E$, Initial model weights: $\theta^{0}$
 
 \FOR{$t=0$ {\bfseries to} $R-1$}
 \STATE Server sends $\theta^{t}$ to all devices \\
 \FOR{client $k=0$ {\bfseries to} $K-1$}
 %\STATE Client k does adversarial training on its local dataset \\
  \STATE $\theta^{t}_{k}$ = \at(E, $\theta^{t}$, $A_{T, \epsilon, \alpha}$) \\
  \STATE Send $\theta^{t}_{k}$ back to server \\
 \ENDFOR
 \STATE \COMMENT {Server performs aggregation over agent updates} \\ $\theta^{t+1} = F(\theta_1^t, \theta_2^t, \ldots, \theta_K^{t})$ \\
 \ENDFOR
  \end{algorithmic}
  \label{algo:FedAT}
\end{algorithm}

\input{fedavg-adv-train}
\input{fedcurv-adv-train}
%We evaluate the efficacy of \fedavgat and \fedcurvat for adversarial training and identify parameters that affect the performance of these algorithms. 

%\textcolor{red}{Supriyo: we do not propose these fusion algorithm. Simply use them as baseline with FAT.}
 %This results in the following objective function
 %$$ \min_{\theta} \rho(\theta); \ \ \ \rho(\theta) = |D_i|/|D| \sum \limits_{k=1}^{K}   \E_{(x,y) \in D_{k}} [\max_{\norm{\Tilde{x}-x}_{\infty} \leq \epsilon} \Lagr(f_{\theta}(\Tilde{x}), y)]$$ 
 %where there are $K$ participating clients, $D_{k}$ is the local dataset at client $k$, $f_{\theta}$ is the deep learning model parameterized by $\theta$ and $\Tilde{x}$ is an $\epsilon$-ball $l_{\infty}$ adversarial sample of benign sample $x$ with class label $y$ ({\bf not clear}).
% \textcolor{red}{Supriyo: Need to rewrite the formulation for FAT using $|D_i|/|D|$ instead of $1/K$}

% %We consider the following baseline in this setting
% \subsection{Local adversarial training}
% Each client performs adversarial training on its local dataset to obtain a robust local model. This approach gives sub-optimal results compared to centralized adversarial training when the amount of data at the client is small or the local data has an uneven distribution of classes relative to the test distribution. Consequently a client's local model cannot reap the benefits of a shared model trained using the combined data of other clients. 


% \begin{algorithm}[]
% \small
% \SetAlgoLined
% \KwIn{
% \begin{enumerate}
%     \item[] PGD Attack: $A_{T, \epsilon, \alpha}$
%     \item[] number of local training epochs: $E$
%     \item[] Initial model weights: $\theta^{0}$
% \end{enumerate}}
% $\theta = \theta^{0}$ \\ 
% Local dataset is (X,Y) \\
% \State \For {$E$ epochs, \forall $x, y \in \{X, Y\}$} 
% {
%     $\Tilde{x} = A_{T, \epsilon, \alpha}(x)$ \\
%     Update $\theta$ to minimize the loss function $\Lagr(f_{\theta}(\Tilde{x}), y)$ between the model output $f_{\theta}(\Tilde{x})$ and groundtruth label $y$ 
% }
% \State \Return $\theta$
%  \caption{\small \textbf{Local adversarial training}}
%  \label{Local_adversarial_training_algo}
% \end{algorithm}

% We report the results on CIFAR10 dataset and the Network-in-Network architecture in \ref{local_adv_training} \textcolor{red}{Supriyo: Delete this and fold into one single description of FAT. Not sure what Table 1 is trying to highlight. Why are we reporting numbers at individual clients. It can confuse the reviewers. We will only report numbers at the server, unless an expt. is explicitly designed to highlight effect on clients.}


%% Problem definition and motivate the approach 
%% Local adversarial training followed by fusion

% Different fusion algorithms: 
% FedAvg, FedCurvature
%Motivate why we are exploring two different fusion algorithms. Talk about IID and non-IID, failure of Fedavg for iid and use of fedcurv for non-iid. 
%% \subsubsection{FedAvg algorithm}
% FedAvg \cite{mcmahan2016communicationefficient} is a widely used algorithm for federated learning. It involves several rounds of communication between the aggregator and the clients. At the beginning of round t, the aggregator sends the model weights $w^{t}$ to each client. Each client trains on its local dataset for $E$ epochs. At the end of round t, each client sends back its updated model weights to the aggregator. The role of the aggregator as the name suggests, is to aggregate the updated model weights from each client. The aggreagtion here is a simple weighted averaging, with each client's update weighed by the number of training data samples at that client.
% Motivate FedAvg for adversarial training with the figure from FedAvg paper
%%Talk about the two baselines: centralized and local adversarial training 



%  \KwIn{
% \begin{enumerate}
%     \item[] number of clients: $K$
%     \item[] number of communication rounds: $R$
%     % \item[] number of steps for PGD attack: $T$
%     % \item[] ball size for PGD Attack perturbation: $\epsilon$
%     % \item[] step-size for PGD Atack: $\alpha$
%     \item[] PGD Attack: $A_{T, \epsilon, \alpha}$
%     \item[] Initial model weights: $\theta^{0}$
%     \item[] number of local training epochs per round: $E$
% \end{enumerate}}
% \For{$t \gets 0$ to $R-1$}{
%     \State Server sends $\theta^{t}$ to all devices \\

%     \State \For {each device k $\in$ \{0...K-1\}}{
        % \State $\theta^{t}_{k}$ = LocalAdversarialTraining(E, $\theta^{t}$, $A_{T, \epsilon, \alpha}$) \\
%         %Write sub-routine for LocalAdversarialTraining
%         % \State \For {$E$ epochs, batch $x_{k}, y_{k} \in \{X_{k}, Y_{k}\}$} 
%         % {
%         %     $\Tilde{x}_{k} = A_{T, \epsilon, \alpha}(x_{k})$ \\
%         %     Update $\theta^{t}_{k}$ to minimize the loss function $\Lagr(f_{\theta^{t}_{k}}(\Tilde{x}_{k}), y_{k})$ between the model output $f_{\theta^{t}_{k}}(\Tilde{x}_{k})$ and the actual label $y_{k}$ 
%         % }
%         \State Send $\theta^{t}_{k}$ back to server
%     }
    
%     \State Server aggregates the client model weights to obtain $\theta^{t+1} = Fusion(\forall_{k \in \{0...K-1\}} \theta^{t}_{k})$
%   }

% \subsection{Dataset and architecture for evaluation}
% We conduct our experiments with two datasets: CIFAR-10 and EMNIST Balanced \cite{cohen2017emnist}. 

% We use Network-in-Network (NIN) \cite{} and VGG-9 \cite{} for training on the CIFAR-10 dataset. 
% For experiments with EMNIST, we use a network with 2 convolution layers followed by 2 fully connected layers. We refer to it as EMNIST-M in subsequent sections.

==> Adversarial training in communication constrained federated learning/svcca_analysis.tex <==
%\subsection{SVCCA Analysis for Model Drift}

%\textcolor{red}{AV: need to discuss the next sentence, does it contradict claim in Fig. 1 in anyway or at least counter to}
%Furthermore, while the adversarial samples constitute effective attacks against the local model, they might not be as effective against the global model. This can negatively impact the overall robustness of the global model. We  validate our hypothesis more formally in the following. 

 Singular Vector Canonical Correlation Analysis (SVCCA) \cite{raghu:svcca} is a technique to compare two network representations that is invariant to affine transforms. SVCCA interprets each neuron as a vector (formed by considering the neuron activations on the input data points) and a layer as subspace spanned by that layer's neurons. 
 
 %We apply this technique to compare the model drift between individual client models in non-iid data setting. 
 We measure the SVCCA scores (in range [0-1]) between the corresponding layer of two models. A high score implies similar representations of two layers (or lower drift), and low score implies that the two layers have learnt different representations (indicating a higher drift). We show results for (i) dependence of model drift on $E$ (ii) comparison of model drift with and without \at in federated learning; and (iii) improvement in model drift due to \feddynat over \fedcurvat and \fedavgat.

% We use five client non-iid data distribution, and select two out of the five NIN models for conducting the analysis. 
% NIN  has  9  convolutional  layers  numbered Conv1...Conv9 with Conv1 being closest to the input layer and Conv9 closest to the output layer. We compute SVCCA scores for four different convolution layers (Conv5...Conv8). Corresponding layers closer to the input (Conv1..Conv4) show less model drift overall.
We report results for two of the five client NIN models\footnote{NIN model: x $\rightarrow$ conv1 $\rightarrow \ldots \rightarrow$ conv9 $\rightarrow$ fc $\rightarrow$ y}. The plots show SVCCA scores for convolution layers $5-8$ where the drift is more pronounced. Layers $1-4$, act as feature extractor layers and show relatively low drift.

%\subsubsection*{Increased Model drift with higher E} \label{svcca_model_drift_dependenceE}
\noindent{\bf Increased model drift with higher E:} With a higher value of $E$, local models train more on local data, consequently the model drift is higher. We illustrate the model drift phenomenon in Fig.~\ref{fig:svcca_E_20_50}, by running \fedavgat with $E=20$ and $E=50$. The SVCCA scores with $E=20$ are much higher than those for $E=50$, indicating a lower model drift for $E=20$.

\begin{figure}[t]
\centering
\includegraphics[scale=0.5]{aaaitoolkit/svcca_E_20_50.png} 
    \caption{\centering \small SVCCA scores evaluated on 2 out of 5 clients for \fedavgat with $E=20$ and $E=50$ using NIN.}
    \label{fig:svcca_E_20_50}
\end{figure}

%\subsubsection*{Comparing Model Drift for \fedavg and \fedavgat on non-iid data} 
\noindent{\bf Comparing model drift with \fedavg and \fedavgat on non-iid data:} In Fig.~\ref{fig:svcca_natural_adversarial.png}, we compute SVCCA scores for \fedavg(natural training) and \fedavgat with $E=50$. We observe that the similarity scores for \fedavgat are generally lower than \fedavg indicating higher drift between the layers. This shows that the drift is higher for adversarial training. 
Furthermore, this drift is more prominent in the higher layers of the model (close to the output). %The layers closer to the input have not been shown in the plots as they show low model drift for both \fedavg and \fedavgat. 

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.5]{aaaitoolkit/svcca_natural_adversarial.png}
    \caption{\centering \small SVCCA scores with $E=50$ for both adversarial and natural training with NIN.}
    \label{fig:svcca_natural_adversarial.png}
\end{figure}

%\subsubsection*{Comparing Model Drift between \feddynat, \fedavgat, \fedcurvat  for non-iid data}
\noindent{\bf Comparing model drift between \feddynat, \fedavgat, \fedcurvat for non-iid data:} In Fig.~\ref{fig:svcca_fedavg_fedcurvature}, we present a comparison of SVCCA scores for \fedavgat, \fedcurvat and \feddynat, all the three techniques we used for adversarial training.
We observe that the similarity score for \fedcurvat is significantly higher than \fedavgat, which validates the proposition that \fedcurvat arrests the local model drift. 

However, \feddynat is able to beat both \fedcurvat and \fedavgat in SVCCA scores. use a constant $E=50$ for local training. \feddynat uses $E_{0}=50, \gamma=0.5, F_{E}=5$ for the E-schedule. As training progresses, and the value of $E$ decreases, less epochs of local model training contributes to a lower model drift. The layers closer to the input have not been shown in the plots as they show low model drift for all 3 algorithms.

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.5]{aaaitoolkit/svcca_fedavg_fedcurvature.png}
    \caption{\centering \small SVCCA scores evaluated on 2 out of 5 clients for \fedavgat, \fedcurvat and \feddynat with NIN. \fedcurvat and \fedavgat use a constant $E=50$ for local training. \feddynat uses $E_{0}=50, \gamma=0.5, F_{E}=5$ for the dynamic E-schedule.}
    \label{fig:svcca_fedavg_fedcurvature}
\end{figure}


==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

Federated learning is a paradigm for multi-round model training over a distributed dataset~\cite{mcmahan2016communicationefficient, kairouz:open}. At the beginning of every round, the participating clients obtain the most recent model from a central server. Clients use the model to perform multiple epochs of local training and share only the parameter updates with the server. The server, in turn, employs a \textit{fusion} algorithm to aggregate the updates from the various clients and generate a new model for the next round. While federation allows the clients to retain control and privacy of their raw data~\cite{bonawitz:secure, truex:privacy}, the final model continues to remain vulnerable to carefully crafted adversarial examples~\cite{szegedy:intriguing, carlini:c_and_w, goodfellow2015explaining} designed to elicit misclassification at inference time. Complementary to our research, there exists a significant body of work on defenses (both empirical~\cite{madry2018towards} and certifiable~\cite{raghunathan:certify, cohen:smoothing}) against adversarial attacks for centralized model training. Among them, adversarial training~\cite{madry2018towards} (\at), formulated as an optimization of the \emph{saddle point problem}, has emerged as the method of choice for training robust models. In this paper, \emph{we study the feasibility of adopting AT to the federated learning setting for training robust models, under realistic constraints on both the client data distribution (non-iid) and the maximum number of possible communication rounds.}

To optimize the minimax objective, \at typically uses multiple iterations of a two-step sequential process: (i) Use Projected Gradient Descent (PGD) to maximize the loss and generate adversarial counterparts for every sample in the training data; (ii) Use Stochastic Gradient Descent (SGD) to optimize the model parameters and minimize the expected loss over the adversarial examples. From an optimization perspective, an immediate consequence of adopting AT to the federated setting is a distributed solution to the minimax objective. In other words, the above two steps, which were earlier performed over the entire data, are now distributed across multiple clients and performed on their local data. Our goal is to design a fusion algorithm, which over multiple rounds ensures that the aggregate model has \emph{comparable} performance in terms of both natural accuracy (measured on benign test samples) and adversarial accuracy (measured on adversarial test samples) w.r.t the model trained in the centralized setting. 
As a first step towards feasibility analysis, we reproduce the observation in  ~\cite{mcmahan2016communicationefficient} for adversarial training. We perform weighted averaging of adversarially trained models from two clients. The models are trained on an iid distributed subset of CIFAR10 data, starting from a common initialization. 
The result shown in Fig.~\ref{fig:feasibility} provides initial evidence that the aggregate model leads to a significant reduction in the loss on the entire training set for both natural and adversarial samples compared to either client models (extreme values of $w$). This implies that fusion can also improve adversarial accuracy (\fedavg had established that fusion helps for natural training).

\begin{figure}[!ht]
\centering
\includegraphics[scale=0.4]{aaaitoolkit/Common_Initialization.png} 
\caption{\centering \small{Loss on CIFAR-10 training set (natural and adversarial samples) using aggregate models. The aggregate model parameters $\theta = w \theta_1 + (1 − w) \theta_2$, where $\theta_1$ and $\theta_2$ are client model parameters, with common initialization but updated independently using local \at at the clients. Mixing weights $w \in [−0.2, 1.2]$.}}
\label{fig:feasibility}
\end{figure}

% Adversarial training works by generating an adversarial counterpart for every sample in the training data (using Projected Gradient Descent, PGD) and then optimizing the model parameters (using Stochastic Gradient Descent, SGD) to minimize the expected loss over the generated samples. Over multiple iterations the model parameters converge to a good solution measured in terms of natural (accuracy on benign test samples) and adversarial (accuracy on adversarial test samples) accuracies. An immediate consequence of adopting AT to federated setting is a distributed solution to its minimax objective. Each client performs local adversarial training on its own dataset and shares the parameter updates with the server. Our goal is to design a fusion algorithm, which over multiple rounds ensures that the aggregate model show improvement in terms of both natural and adversarial accuracies. As a first step towards feasibility analysis, we used \fedavg~\cite{mcmahan2016communicationefficient} as a fusion algorithm with AT performed at each of the clients. Fig.~\ref{fig:feasibility} provides evidence that fusion can also benefit adversarial accuracy (earlier \fedavg had established that fusion helps with natural accuracy). In other words, the aggregate model obtained after fusion has better adversarial accuracy compared to the individual updates.
% \begin{figure}[!ht]
%     \centering
% \includegraphics[width=1.0\columnwidth]{aaaitoolkit/Common Initialization.png} 
%     \caption{The loss on the full CIFAR10 training set (on natural and adversarial samples) for models generated by averaging the parameters of two models $\theta$ and $\theta^{'}$ using $w \theta + (1 − w) \theta^{'}$ for 50 evenly spaced values $w \in [−0.2, 1.2]$. The models $\theta$ and $\theta^{'}$ were initialized with the same weights and adversarially trained using SGD on different small datasets. As we see from the figure, averaging the models produces a significant reduction in the loss on the total training set for both natural and adversarial samples much better than the loss of either parent model.}
%     \label{fig:feasibility}
% \end{figure}

\noindent{\bf Challenges:} However, there are several challenges that need to be addressed. Using centralized clean training as baseline, we observed a higher drop in both natural and adversarial accuracies when \at is used in the federated setting as opposed to centralized training. We attribute this to number of epochs of local AT, denoted by $E$, performed at each client, which in turn causes the local models at the clients to \textit{drift} further from each other. This is over and above the drift that is already introduced by the non-iid data distribution at the clients. We use SVCCA~\cite{raghu:svcca} scores to quantify model drift across clients.  In addition, the convergence time (in terms of the number of communication rounds) is also increased. This is of particular concern as it increases the communication cost significantly.

\noindent{\bf Contributions:}
Towards this end, we propose \feddynat, which builds on the techniques proposed for preventing catastrophic forgetting in federated learning on non-iid data~\cite{shoham2019overcoming, kirkpatrick2016overcoming} by augmenting them with a dynamic local AT schedule ($E$-schedule). We make the following contributions..

\begin{itemize}[noitemsep,nolistsep]
    \item We study the performance of adversarial training in a federated setting with non-iid data distribution and discuss the challenges involved as compared to normal training.
    \item We present a novel algorithm for improving the performance of adversarial training in federated setting with non-iid data distribution, called \feddynat, and evaluate its performance over multiple datasets and models. We compare the performance with other state-of-the art methods used in normal federated learning.
    \item We analyze the performance of different algorithms in the federated setting using model drift across various clients and provide insights on the relative performance.
\end{itemize}


%The dynamic $E$-schedule is motivated by the key insight that on one hand, small values of $E$ require clients to frequently share their model updates with the server. \textcolor{red}{AV: shall we defer this discussion to later as we are not providing any results or substantiating the claims otherwise}This causes the models to drift less, leading to improvement in both adversarial and natural accuracies, but at the cost of increased convergence time. On the other hand, larger values of $E$ causes the models to converge faster, but leads to an overall reduction in accuracy. Specifically, dynamic $E$-schedule in \feddynat is designed to amplify the ability of  \fedcurv~\cite{shoham2019overcoming} to handle model drift while simultaneously encouraging faster model convergence. Through extensive experiments on multiple benchmarking datasets we show that for a fixed budget on the number of communication rounds, \feddynat leads to reduced drift between models (higher similarity), causing an improvement in both natural and adversarial accuracies compared to other fusion approaches. Further, experimentation show that \feddynat performance is robust to the choice of associated hyperparameters, i.e., different dynamic $E$-schedule, satisfying some general requirements, result in very similar performance. 




% \section{Introduction}
% Federated learning is a paradigm for multi-round model training over a distributed dataset. At the beginning of every round, the participating clients obtain the most recent model from a centralized server. clients use the model to perform local training and share only the parameter updates with the server. The server, in turn, employs a \textit{fusion} algorithm to aggregate the updates from the various clients and generate a new model for the next round. While federation allows the clients to retain control and privacy of their raw data~\cite{SecureAggSchemes}, the final model continues to remain vulnerable to carefully crafted adversarial examples~\cite{advAttacks}. 


% \begin{itemize}
%     \item Motivate need for robust models in federated setting. Refer to Supriyo's paper and other pointing why FL brings new dimension to adversarial attacks.  
%     \item talk about adversarial training as a means to achieve robustness however prior work mostly focused on centralized training. 
%     \item Question is to how to do adversarial training in a federated setting. Should the clients just do adversarial training completely locally and synchronize at the very end or the clients should do periodic synchronization while training. It is shown for regular training fusion helps (refer to FedAvg original paper). Then talk about our initial experiment corresponding to Fig. 1.   Refer to Fig.1 showing that for  adversarial training also fusion is helpful.
    
%     \item Talk about challenges associated with FL including non-iid data distribution, communication and convergence tradeoff in federared learning in general. How to effectively design algortihms to deal with non-iidness and leverage tradeoff when designing algorithms for adversarial training in a federated setting.
%     \item Talk about our contributions
% \end{itemize}
% \subsection{Adversarial training}
% Adversarial training is a standard approach to improve the robustness of deep learning models. In adversarial training, the deep learning model is trained with adversarially perturbed samples to improve the robustness of the model on such samples at test-time. There exist a lot of attacks against various types of deep learning models ranging from classification \cite{goodfellow2015explaining} to object detection \cite{xie2017adversarial} and 3D point cloud classification \cite{liu2020adversarial}. The general principle behind an attack is to identify data points in the input space which are imperceptibly close to the training data points, but which maximize the loss function being optimized by the model. The problem formulation is 
% $$ \argmax_{\Tilde{x}} \Lagr(f_{\theta}(\Tilde{x}), y) \ \text{s.t} \ d(x, \Tilde{x}) < \epsilon $$

% where $\Lagr$ is the loss function between the output of the model $f_{\theta}$ and the actual label $y$, $d$ is a distance metric between the original training sample $x$ and the corresponding
% adversarial sample $\Tilde{x}$ and $\epsilon$ is a predetermined threshold

% In this work we use a state-of-the-art adversarial training benchmark proposed by \cite{madry2018towards}. It aims to solve the following min-max robust optimization problem,
% $$ \min_{\theta} \rho(\theta); \ \ \ \rho(\theta) = \E_{(x,y) \in D} [\max_{\norm{\Tilde{x}-x}_{\infty} \leq \epsilon} \Lagr(f_{\theta}(\Tilde{x}), y)]$$, where $f_{\theta}$ is the deep learning model parameterized by $\theta$ and $\Tilde{x}$ is an $\epsilon$-ball $l_{\infty}$ adversarial sample of benign sample $x$ with class label $y$ ({\bf not clear}). $\Tilde{x}$ is generated using Projected Gradient Descent (PGD) 
% $$ x^{t+1} = \Pi(x^{t} + \alpa sign(\nabla_{x^{t}} \Lagr(f_{\theta}(x^{t}), y))) $$, where $\alpha$ is the step size and $\Pi(.)$ projects the result of the gradient step into the $\epsilon$-ball around the original sample, $x$.
% %It is a T-step PGD attack. As the value of T increases, the adversaries become stronger resulting in
% %a greater chance of misclassification by the trained model.

% %% Mention the architectures - NIN and VGG-9. Show the final accuracies (no need for graph)%%

% \subsection{Federated learning}
% Talk about Macmahan paper(Fedavg) and Fedcurvature
% Challenge and our contribution

==> relatedWork.tex <==
\section{Related Work}
To address communication overhead in distributed learning, algorithms perform multiple local epochs of training before synchronization and thus reduce the communication overhead~\cite{konecny16,mcmahan2016communicationefficient,NEURIPS2019_4aadd661}. The convergence analysis of these algorithms connects the rate of convergence with number of clients and local training epochs~\cite{yu2019linear,yu2018parallel}. These results are mostly  obtained under strong assumptions on the degree of dissimilarity (i.e., non-iidness) in the data distribution between clients which may not hold in practice. Of particular relevance to our work is~\cite{Wang2019AdaptiveCS} which analyses tradeoff between decreased wall clock time for convergence and increase in convergence error with increasing $E$. Based on the analysis for iid distribution, an adaptive algorithm is proposed that dynamically changes the number of local training rounds. 
%All the results have been proposed and evaluated for natural training only. 
%Recently theoretical analysis has been conducted for unbounded dissimilarity~\cite{}. 

%SeverFederated learning is challenging with non-iid data distribution between clients and 
Several algorithms have been proposed to achieve faster convergence while reducing communication overhead with non-iid data. ~\cite{li2018federated, shoham2019overcoming} use additional regularization terms in the client loss function to minimize divergence between local and global models. 
Going beyond simple averaging of weights during fusion, ~\cite{pmlr-v97-yurochkin19a, wang2020federated} perform layer-wise matching of neurons from different clients, before averaging the model weights leading to improved communication efficiency. To prevent interference between incompatible tasks across clients, ~\cite{yoon2020federated} selectively transfers the knowledge between clients. All the above fusion algorithms have been studied for natural training only.

In centralized setting \at by ~\cite{madry2018towards} is shown to provide some of the strongest defense against PGD attacks~\cite{pmlr-v80-athalye18a} and is a widely accepted benchmark~\cite{hendrycks2019pretraining, pmlr-v80-athalye18a}. In concurrent work,~\cite{zizzo2020fat} has also implemented traditional \at in federated setting. Different from our work, their focus was on evaluating the vulnerability of both Byzantine resilient defenses and federated \at, rather than mitigating the performance impact of \at in federated setting.  




